Ethical Reasoning over Moral Alignment: A Case and Framework for In-Context Ethical Policies in LLMs

In this position paper, we argue that instead of morally aligning LLMs to specific set of ethical principles, we should infuse generic ethical reasoning capabilities into them so that they can handle value pluralism at a global scale. When provided with an ethical policy, an LLM should be capable of making decisions that are ethically consistent to the policy. We develop a framework that integrates moral dilemmas with moral principles pertaining to different foramlisms of normative ethics, and at different levels of abstractions. Initial experiments with GPT-x models shows that while GPT-4 is a nearly perfect ethical reasoner, the models still have bias towards the moral values of Western and English speaking societies.

==> 01_examples.tex <==
\subsection{Applications of RAI}
\subsubsection{Chatbots}
 In the case of a chatbot, we can identify two sources of harms -- namely user offense, wherein the user propagates harms in their conversation, or bot-offense, where the chatbot emits harmful content to a user. It is imperative that each of these sources be handled differently -- i.e. the user may handle a harm differently as compared to a bot. For instance, it is completely fine if a user provides ungrounded advice to a bot. For example uttering the following statement to a chatbot is perfectly reasonable: \\

\texttt{I think you should break-up with your creators.}\\
However, a bot may not advise the user to break-up with their creator(s).\\
It is also possible to adversarially generate offensive statements by red-teaming language models \cite{perez-etal-2022-red} \cite{ganguli-etal-2022-red}. 

\subsubsection{Text-prediction scenarios}
Text-prediction models have been shown to exhibit biases [CITE EACL paper], and  influence users based on their own biases [CITE ADVAITH PAPER]. This is especially true in the case of long-form text prediction which involves the prediction of multiple words as opposed to filling in characters.
For example:\\

\texttt{My favorite country is The U\color{gray}nited Kingdom.\color{black}} \\

can be biased -- since the user could also be intending to type `The United states of America' instead.

In both cases, the definition of harms varies vastly, and as a result, each application would require independent data collection, annotation, and training.\\ 


